PacGAN: The power of two samples in generative adversarial networks

Generative adversarial networks (GANs) are innovative techniques for learning generative models of complex data distributions from samples. Despite remarkable recent improvements in generating realistic images, one of their major shortcomings is the fact that in practice, they tend to produce samples with little diversity, even when trained on diverse datasets. This phenomenon, known as mode collapse, has been the main focus of several recent advances in GANs. Yet there is little understanding of why mode collapse happens and why existing approaches are able to mitigate mode collapse. We propose a principled approach to handling mode collapse, which we call packing. The main idea is to modify the discriminator to make decisions based on multiple samples from the same class, either real or artificially generated. We borrow analysis tools from binary hypothesis testing---in particular the seminal result of Blackwell [Bla53]---to prove a fundamental connection between packing and mode collapse. We show that packing naturally penalizes generators with mode collapse, thereby favoring generator distributions with less mode collapse during the training process. Numerical experiments on benchmark datasets suggests that packing provides significant improvements in practice as well.

==> ganview.tex <==

% ====================================================
\section{GANView: a dashboard for GAN}
\label{sec:ganview}

As discussed in the theory Section \ref{sec:theory}, for a given pair of distributions $(P,Q)$, the two-dimensional mode collapse region $\mathcal{R}(P,Q)$ precisely characterizes the region of $(\epsilon,\delta)$ such that $(P,Q)$ exhibit $(\epsilon,\delta)$-mode collapse. 
In this section, we seek to numerically estimate this region from the samples generated from the two distributions $P$ and $Q$. We call this numerically estimated region to be {\em GANView} when $P$ is the target distribution and $Q$ is the generator distribution.
Note that our approach to estimate the region $\mathcal{R}(P,Q)$ can be applied to samples generated from any pair of distributions $(P,Q)$. 

There are various ways in which GANView can be helpful in training a GAN. For example, while training we can plot GANView for each epoch and decide early stopping based on when the region has minimal area. We leave these explorations of the use of the GANView for future study. In the following, we give an alternate characterization of the GANView region $\mathcal{R}(P,Q)$ and propose an algorithm to estimate it from the samples.

The GANView region $\mathcal{R}(P,Q)$ can be defined in the following way.
\begin{eqnarray}
\mathcal{R}(P,Q) & \equiv &  \bigcap_{\alpha \in [0,\infty]} \bigg\{ (\epsilon, \delta) :    \epsilon \leq \delta \leq \alpha(\epsilon - Q(S_{\alpha})) + P(S_{\alpha})\bigg\} \, \label{eq:g1}\\
& \equiv & \text{Convex hull} \bigg\{(P(S_{\alpha}), Q(S_{\alpha}))\;\; \text{for} \;\alpha \in [0,\infty] \bigg\}\, \label{eq:g1a}
\end{eqnarray}
where $S_{\alpha}$ is defined to be
\begin{eqnarray}
\label{eq:g2}
S_{\alpha} &\equiv & \arg\max_{S' \in \Omega} \bigg\{ S' : \forall x \in S', \frac{p(x)}{q(x)} \geq \alpha    \bigg\}\,
\end{eqnarray}
where $p(x)$ and $q(x)$ are the densities of the two distributions $P$ and $Q$ respectively. 

Based on the above definition of $\mathcal{R}(P,Q)$ it is immediate that by estimating $P(S_{\alpha})$ and $Q(S_{\alpha})$ for various values of $\alpha$ in $[\infty, 0]$, we can estimate the mode-collapse region. 
For estimating $P(S_{\alpha})$ and $Q(S_{\alpha})$, we propose the following approach. 
For each $\alpha$, we learn a binary classifier $G_{\alpha}$ with a suitably modified loss function. We use a 
weighted cross-entropy loss function which gives an unbiased estimate of  $P(S_{\alpha})$ and $Q(S_{\alpha})$. In particular, $G_{\alpha}$ minimizes the following loss function:
\begin{eqnarray}
\label{eq:g3}
G^{*}_{\alpha} & \equiv & \arg\min_{G} \Bigg\{ \frac{1}{\alpha + 1}\mathbb{E}_{x \sim p(x)} \big[\log(G(x)) \big] + \frac{\alpha}{\alpha + 1}\mathbb{E}_{x \sim q(x)} \big[\log(1 - G(x)) \big] \Bigg\}\,,
\end{eqnarray}
where the classifier $G(x) \in [0,1]$.
\begin{propo} 
The optimal classifier $G^{*}_{\alpha} $ is:
\begin{eqnarray}
\label{eq:g4}
G^{*}_{\alpha} (x) = \frac{p(x)}{p(x) + \alpha q(x)}\,.
\end{eqnarray}
\end{propo}
Using the classifier $G^{*}_{\alpha} (x)$, we can estimate $P(S_{\alpha})$ and $Q(S_{\alpha})$ in the following way.
\begin{eqnarray}
\label{eq:g5}
P(S_{\alpha})  & = & \mathbb{E}_{x \sim p(x)} \left[\mathbb{I}(G^{*}_{\alpha} (x) \geq 1/2) \right]\, \\
Q(S_{\alpha})  & = & 1 - \mathbb{E}_{x \sim q(x)} \left[\mathbb{I}(G^{*}_{\alpha} (x) < 1/2) \right]\,.
\end{eqnarray}

By learning the optimal classifier $G^{*}_{\alpha} (x)$ for multiple values of $\alpha \in [0,1]$, and estimating  $P(S_{\alpha})$ and $Q(S_{\alpha})$ numerically using Equation \eqref{eq:g5}, we can estimate the region $\mathcal{R}(P,Q)$. However, due to finite samples, the numerically estimated values of $P(S_{\alpha})$ and $Q(S_{\alpha})$ may not be consistent for different $\alpha$ values, and the resulting mode-collapse region $\mathcal{R}(P,Q)$ drawn using Equation \eqref{eq:g1}. Therefore, we use the definition of  $\mathcal{R}(P,Q)$ in Equation \eqref{eq:g1a} to estimate the region. 
 
Based on the above discussions we present Algorithm 1 to estimate GANView region $\mathcal{R}$ using the samples generated from the two distributions $P$ and $Q$.
Given $n$ samples from each of the two distributions $P,Q$, and a set of $K$ $\alpha$ values for $\alpha \in [0,\infty]$, Algorithm \ref{algo:ganview} returns an estimate of mode-collapse region $\widehat{\mathcal{R}}(P,Q)$ which approaches the true region $\mathcal{R}(P,Q)$ as the number of samples $n$ goes to infinity. We use $n/2$ samples of each distribution to learn the binary classifier $G^{*}_{\alpha}$ and the remaining samples to estimate the probabilities $P(S_{\alpha})$ and $Q(S_{\alpha})$, for each value of $\alpha$. 

\begin{algorithm}[ht]
\caption{GANView}
\label{algo:ganview}
  \begin{algorithmic}[1]
    \REQUIRE $P$: ${\{X_i\}}_{i \in [n]} \sim P$, ${\{Y_j\}}_{j \in [n]} \sim Q$, a set of positive numbers  ${\{\alpha_k\}}_{k \in [K]}$
	\ENSURE $\widehat{\mathcal{R}}(P,Q)$
	\FOR{$k = 1$ to $K$} 
	\STATE $\alpha = \alpha_k$
	\STATE $G^{*}_{\alpha}  =  \arg\min_{G} \bigg\{\sum_{i=1}^{n/2}\big[\log(G(X_i)) \big] + \alpha \sum_{j=1}^{n/2}\big[\log(1 - G(Y_j))\big] \bigg\}\,,$
	\STATE $P(S_{\alpha})   = \frac{2}{n} \sum_{i=n/2+1}^{n} \mathbb{I}(G^{*}_{\alpha} (X_i) \geq 1/2) \,$
	\STATE $Q(S_{\alpha})  = 1 - \frac{2}{n} \sum_{j=n/2+1}^{n} \mathbb{I}(G^{*}_{\alpha} (Y_j) < 1/2) \,$
	\ENDFOR   
	\STATE $\widehat{\mathcal{R}}(P,Q) =  \text{Convex hull} \bigg\{(P(S_{\alpha}), Q(S_{\alpha}))\;\; \text{for} \;\alpha \in [0,\infty] \bigg\}$
      \end{algorithmic}
\end{algorithm}


%The following theorem gives a sample complexity bound on the accuracy of the estimation of each of the points $P_{\alpha}(S)$ and $Q_{\alpha}(S)$ for any alpha in $[\infty,0]$.
%
%Numerical results:
%explain the setting of the binary classifier: multi-layer perceptron of depth 2 with each layer having $500$ nodes, 
%We show numerical experiments on plotting GANView for the settings presented in the Numerical Experiments section. 
%
%DISCRIMINATOR AS ESTIMATOR!!! 
%
%
%1. motivation: TensorBoard \cite{AABB16} 
%2. challenge: visualization from samples
%3. solution: 
%4. results: (2D, GANView)-iterations[DCGAN], (2D, GANView)-iterations[PACGAN] 
%
\begin{figure}[ht]
	\begin{center}
	\includegraphics[width=.9\textwidth]{gan_view_figures/gauss_grid_1}
	\includegraphics[width=.9\textwidth]{gan_view_figures/gauss_grid_2}
	\end{center}
	\caption{GAN View plots for 2D gaussian mixture over epochs starting from 1 to 400. Epoch numbers increase in row. Bottom right figure corresponds to epoch number $400$. GAN-1 and GAN-2 are fairly monotonous. However, GAN-3 and GAN-4 show a significant fluctuation.}
	\label{fig:GANView1}
\end{figure}

 1 - p(s) + alpha q(s)
%
%\begin{figure}[ht]
%	\begin{center}
%		% D1,D2,D3,GV
%	\end{center}
%	\caption{}
%	\label{fig:GANView2}
%\end{figure}
%
%\begin{figure}[ht]
%	\begin{center}
%		% D1,D2,D3,GV
%	\end{center}
%	\caption{TV vs. mode-collapse, over iterations, for multiple architectures.}
%	\label{fig:GANView3}
%\end{figure}





==> section2.tex <==

% ================================================================
\section{PacGAN: A framework for mitigating mode collapse}
\label{sec:pacgan}

We propose a new framework for mitigating mode collapse in GANs. 
Suppose we start with a fixed GAN with our choices of a generator architecture, a discriminator architecture,  
and a loss function. 
Let us call this baseline a mother architecture. 
The framework of PacGAN is to maintain the same generator architecture and the loss function as the mother architecture, 
and make a slight change only in the discriminator. Hence, the overhead is light in the changes made to the architecture and also in the additional computational complexity. 




The key idea of PacGAN is the following:  instead of letting the discriminator $D(X)$ take in a single sample (from real data or from the generator), we make slight changes to the discriminator $D(X_1,X_2,\ldots,X_m)$ to take in 
 $m$ concatenated independent samples from the same distribution---either  real (jointly labelled as $Y=1$) or generated (jointly labelled as $Y=0$). 
%These concatenated samples are either all real or all generated, and 
We refer to the concatenation of samples with the same label as {\em packing}, 
and the resulting concatenated discriminator as {\em packed discriminator}, 
and the number $m$ of concatenated samples as the {\em degree of packing}. 
We call this approach a framework instead of an architecture,
 because the proposed approach of packing can be applied to 
any existing GAN, using any architecture and any loss function, as long as it uses a discriminator of the form $D(X)$ 
which classifies a single input sample.  

We propose the nomenclature  ``Pac(X)($m$)'' where 
(X) is the name of the mother architecture, and 
($m$) is an integer that refers to how many samples are packed together as an input to the discriminator.
For example, if we take an original GAN and feed the discriminator three packed samples as input, 
we call this ``PacGAN3''. % which we used to get the results in Table \ref{tbl:veegan1}. 
If we take the celebrated DCGAN \cite{RMC15} and feed the discriminator four packed samples as input, 
we call  this ``PacDCGAN4''. % which we used to get the results in Table \ref{tbl:veegan2}.
%This setup is illustrated in Figure \ref{fig:framework}.
When we refer to the generic principle of packing, we use PacGAN without an subsequent integer.


Note that there are many ways to change the discriminator architecture to accept packed input samples.
%In our experiments, we use a naive approach of keeping all the layers exactly the same as the mother architecture, 
%while simply making the input space $m$ times larger, resulting in $m$ times more weights in the first layer. 
We propose keeping all hidden layers of the discriminator exactly the same as the {\em mother} architecture that PacGAN is building upon, 
and only increasing the number of nodes in the input layer by a factor of $m$. 
Hence, the computational overhead in implementing PacGAN is marginal; 
the number of parameters in the discriminator increases only marginally. 
For example, if we are modifying an original GAN, the input layer would be expanded by a factor of $m$, as would the number of edges in the first fully-connected layer. 
For DCGAN, we simply stack the images into a tensor of depth $m$;
for instance, the discriminator for PacDCGAN5 on the MNIST dataset of handwritten images \cite{mnist} would take an input of size $28\times28\times 5$ (each individual black-and-white image is $28\times 28$ pixels). %, as each image has RGB dimensions and there are three such dimensions  stacked. 
By modifying only the input dimension, we can focus purely on the effects of the proposed concept of {\em packing}. 
%It is also possible to search over the space of possible ways to pack samples, 
%but we leave this question as a direction for future research. 

Further, there is no additional hyper-parameter tuning required, as we keep {\em all} the hyper-parameters  in training 
the same as those used in the mother architecture (on top of keeping the architecture almost the same), including 
size of mini-batch in stochastic gradient descent, weight decay, learning rate, and the number of epochs.
This should be contrasted with other approaches to  mitigate mode collapse that 
require significant computational overhead and/or delicate choice of hyper-parameters \cite{DBP16,DKD16,SGZ16,SVR17,MPP16}. 


Just as in the standard GAN, a bag of samples from the real data and the generator is used to train the packed discriminator. 
Each mini-batch in the stochastic gradient descent now consists of 
several {\em packed} samples, where each packed sample is of the form  
$(X_1,X_2,\ldots,X_m,Y)$, where the label $Y$ is one for real data and zero for generated data, 
and $m$ independent samples from that class is jointly treated as a single higher dimensional feature $(X_1,\ldots,X_m)$. 
%$m$ packed samples from the same distribution $(X_1,X_2,\ldots,X_m)$ (either from the generator or the real data) 
%and the label $Y$ (zero for generator and one for the real data).
%Upon receiving these concatenated samples, the discriminator classifies the batch of $m$ samples jointly, as real or generated. 
The discriminator learns to classify $m$ packed samples jointly. 
Intuitively, this packing allows the discriminator to easily detect mode collapse, as lack of diversity is easier to detect when you look at multiple samples jointly. 
Fundamentally, we are allowing the discriminator the power to look at samples from the product distribution. 
This  allows the discriminator the power to discriminate mode collapsing generators, as we make precise in Section \ref{sec:theory}.




%%\begin{wrapfigure}[15]{R}{0.4\textwidth}
%\begin{figure}[ht]
%%    \centering
%\begin{center}
%  \includegraphics[width=0.3\textwidth]{figures/framework}
%%  \put(-215,30){\rotatebox{90}{Probability of Detection}}
%%  \put(-120,-10){Tree degree, $d$}
%\end{center}
%  \caption{The proposed packing framework can be integrated into any GAN architecture and loss function. {\bf can we change packing factor to degree of packing?}}
%  \label{fig:framework}
%  \end{figure}
%%\end{wrapfigure}



\paragraph{Computational complexity.} 
Packing marginally increases the computational complexity of GAN training. 
The exact increase is architecture-dependent, but can be computed in a straightforward manner.
For example, consider a discriminator with $w$ fully-connected layers, each containing $g$ nodes. 
Since the discriminator has a binary output, the $(w+1)$th layer has a single node, and is fully connected to the previous layer.
We seek the computational complexity of a single minibatch parameter update, where each minibatch contains $r$ samples. %data elements. 
Backpropagation in such a network is dominated by the matrix-vector multiplication in each hidden layer, which has complexity $O(g^2)$ per input sample, assuming a naive implementation.
Hence the overall minibatch update complexity is $O(rwg^2)$.
Now suppose the input layer is expanded by a factor of $m$.
%The input layer now dominates the overall computational cost.
If we keep the same number of minibatch elements, the per-minibatch cost grows to $O((w+m)rg^2)$. 
%increasing by a factor of $\frac{m}{w}$ if $m>w$, and 1 otherwise. 
We find that in practice, $m=2$ or $m=3$ give good results. % and the depth of the discriminator dominates this asymptotic complexity.
%However, the total number of real data samples remains constant, so the number of minibatches per epoch is reduced by a factor of $m$.
%However, in principle, one could also keep the number of total samples constant even as the packing factor grows, so the number of minibatch elements is reduced to $r/m$. 
%This adjustment keeps the per-epoch complexity unchanged.
%This back-of-the-envelope approximation will typically be loose in practice, particularly for discriminators with a deep architecture. 
%We discuss the empirical training runtime  more in Section \ref{sec:exp}. {\bf shouldn't $r$ decrease by a factor of $m$?}


